Legendrian knots, transverse knots and combinatorial Floer homology

Using the combinatorial approach to knot Floer homology, we define an invariant for Legendrian knots in the three-sphere, which takes values in link Floer homology. This invariant can be used to also construct an invariant of transverse knots.

==> draws/munge-filenames <==
#!/bin/sh
# This is really horrible hackery to get MetaPost output to have the
# right extension

for f in `find . -name $1.\[0-9\]\*`
do  g=`echo $f | sed 's/\.\([0-9]*\)$/-\1.eps/'`
    mv $f $g
    ln -s $g ${g%.eps}.mps
done
